Gradient Obfuscation Checklist Test Gives a False Sense of Security

One popular group of defense techniques against adversarial attacks is based on injecting stochastic noise into the network. The main source of robustness of such stochastic defenses however is often due to the obfuscation of the gradients, offering a false sense of security. Since most of the popular adversarial attacks are optimization-based, obfuscated gradients reduce their attacking ability, while the model is still susceptible to stronger or specifically tailored adversarial attacks. Recently, five characteristics have been identified, which are commonly observed when the improvement in robustness is mainly caused by gradient obfuscation. It has since become a trend to use these five characteristics as a sufficient test, to determine whether or not gradient obfuscation is the main source of robustness. However, these characteristics do not perfectly characterize all existing cases of gradient obfuscation, and therefore can not serve as a basis for a conclusive test. In this work, we present a counterexample, showing this test is not sufficient for concluding that gradient obfuscation is not the main cause of improvements in robustness.

==> latex/paper/05_discussion.tex <==
\section{Discussion}

Gradient obfuscation is a problem when it comes to determining the robustness of a model. However, when it comes to just defending against adversarial attackers, there are scenarios when gradient obfuscation can be viewed as more of an attribute, than a weakness.
Firstly, performing the EoT gradient estimation inside an attack is usually significantly more computationally demanding than the regular attack, making the attack itself more difficult to perform.
Secondly, the attacker might be oblivious to the presence of the noise in the model, and therefore they might not use the EoT estimation. In the case of PNI, the noise scaling coefficient $\alpha_i$ can be tuned by the user instead, thus the architecture would remain the same, which would make the presence of noise in the model more difficult to detect.
Furthermore, there are scenarios where the attackers deploy universal adversarial examples, designed to fool various different models at once, instead of tailoring the attacks to the specific model/defense.
Finally, the defense designer can attempt to design noise distributions and methods, which make the gradient estimation more difficult.

==> tables/paper/PNI_transformer_100_FAIL.tex <==
\begin{table}[t]
\centering
\tableFont
\captionsetup{font=small}
\caption{\textbf{asdaI}. asdas
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\resizebox{\columnwidth}{!}{
%\renewcommand\arraystretch{1}
%\resizebox{\columnwidth}{!}{


\centering
\begin{tabular}{|c||c|c|c|c|c|}

\hline
& \multicolumn{5}{c|}{\makecell{Accuracy $\uparrow$}} \\ \cline{2-6}
 
& \makecell{Clean \\ samples}
& {\makecell{FGSM \\ attack}} 
& {\makecell{FGSM \\ attack \\ (EoT$-5$)}} 
& {\makecell{PDG$-10$ \\ attack}} 
& {\makecell{PDG$-10$ \\ attack \\ (EoT$-5$)}} 
\\  \hline \hline 
  
& \multicolumn{5}{c|}{\makecell{Adversarial fine-tuning with $\epsilon=\frac{2}{255}$}} \\ \hline \hline

DeiT-S 
& $75.28\%$ & \multicolumn{2}{c|}{$59.94\%$} & \multicolumn{2}{c|}{$53.26\%$} \\ \hline 

\makecell{ DeiT-S + PNI-W-fc2 \\(layerwise)}
& $75.00\%$ & $60.24\%$ & $60.20\%$ & $53.88\%$ & $53.84\%$ \\ \hline

\makecell{ DeiT-S + PNI-W-fc2 \\(channelwise)}

& $74.66\%$ & $60.06\%$ & $60.18\%$ & $53.32\%$ & $53.20\%$ \\ \hline
 
\makecell{ DeiT-S + PNI-W-fc2 \\(elementwise)}
& $74.62\%$ & $59.42\%$ & $59.28\%$ & $52.82\%$ & $52.52\%$ \\ \hline \hline


& \multicolumn{5}{c|}{\makecell{Adversarial fine-tuning with $\epsilon=\frac{4}{255}$}} \\ \hline \hline

DeiT-S 
& $65.38\%$ & \multicolumn{2}{c|}{$45.58\%$} & \multicolumn{2}{c|}{$37.36\%$} \\ \hline 

\makecell{ DeiT-S + PNI-W-fc2 \\(layerwise)}
& $66.12\%$ & $47.02\%$ & $47.00\%$ & $38.04\%$ & $37.98\%$ \\ \hline

\makecell{ DeiT-S + PNI-W-fc2 \\(channelwise)}
& $66.20\%$ & $46.22\%$ & $46.28\%$ & $38.26\%$ & $38.12\%$ \\ \hline
 
\makecell{ DeiT-S + PNI-W-fc2 \\(elementwise)}
& $65.80\%$ & $46.84\%$ & $46.32\%$ & $37.86\%$ & $37.52\%$ \\ \hline

% Iterations per attack & 0 & 50 & 250 \\ \hline
\end{tabular}
\label{tab:PNI_merged_trf}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\label{tab:PNI_merged}
\end{table}


==> tables/paper/PNI_variants.tex <==
\begin{table*}[t!]
\centering
\tableFont
\captionsetup{font=small}
\caption{\textbf{Abc}. Abc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\resizebox{\columnwidth}{!}{
%\renewcommand\arraystretch{1}
%\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{|c|l||c|c|c|c||c|c|c|c|}

\hline
\multicolumn{2}{|c||}{} & \multicolumn{8}{c|}{\makecell{Accuracy $\uparrow$}} \\ \cline{3-10}
  
\multicolumn{2}{|c||}{} 
 %& Clean
 & \multicolumn{4}{c||}{\makecell{Adversarial training \\ with $\epsilon=\frac{2}{255}$~\cite{Wong2020FastIB} }} 
 & \multicolumn{4}{c|}{\makecell{Adversarial training \\ with $\epsilon=\frac{4}{255}$~\cite{Wong2020FastIB}}}
 \\ \cline{3-10}
 
\multicolumn{2}{|c||}{} 
 & \makecell{Clean \\ samples}
 & {\makecell{FGSM \\ attack}} 
 & {\makecell{PDG$-10$ \\ attack}} 
 & {\makecell{PDG$-10$ \\ with EoT$-25$  \\ attack}} 
 & \makecell{Clean \\ samples}
 & {\makecell{FGSM \\ attack}} 
 & {\makecell{PDG$-10$ \\ attack}}
 & {\makecell{PDG$-10$ \\ with EoT$-25$ \\ attack}} 
 \\ \hline \hline
 
\multicolumn{2}{|c||}{ResNet50} & 
$82.90\%$ & $72.24\%$ & \multicolumn{2}{c||}{$65.44\%$} & $78.12\%$ & $61.72\%$ & \multicolumn{2}{c|}{$50.94\%$} \\ \hline \hline

\multirow{2}{*}{\makecell{ResNet50 + PNI-W \\ (layerwise)}} & 
$\eta \sim \mathcal{N}(0,\sigma^2)$ & $83.16\%$ & $77.60\%$ & $70.26\%$ & $62.70\%$ & $82.02\%$  & $71.24\%$ & $60.60\%$ & $44.50\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$ & $83.02\%$ & $76.04\%$ & $69.62\%$ & $64.00\%$ & $82.18\%$  & $72.86\%$ & $62.54\%$ & $45.16\%$ \\ \hline

\multirow{2}{*}{\makecell{ResNet50 + PNI-W \\ (channelwise)}}
& $\eta \sim \mathcal{N}(0,\sigma^2)$ & $84.50\%$ & $77.62\%$ & $68.92\%$ & $60.02\%$ & $82.54\%$  & $72.68\%$ & $60.38\%$ & $42.62\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$ & $84.32\%$ & $77.50\%$ & $69.70\%$ & $62.06\%$ & $83.42\%$  & $73.54\%$ & $62.46\%$ & $43.42\%$ \\ \hline \hline

\multirow{2}{*}{\makecell{ResNet50 + PNI-A-a\\ (layerwise)}}
& $\eta \sim \mathcal{N}(0,\sigma^2)$ & $85.06\%$ & $75.52\%$ & $66.74\%$ & $59.04\%$ & $82.08\%$ & $67.32\%$  & $55.12\%$ & $42.64\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$ & $84.02\%$ & $72.80\%$ & $63.82\%$ & $54.32\%$ & $79.44\%$  & $62.90\%$ & $50.28\%$ & $36.84\%$ \\ \hline

\multirow{2}{*}{\makecell{ResNet50 + PNI-A-a \\ (channelwise)}}
& $\eta \sim \mathcal{N}(0,\sigma^2)$ & $85.20\%$ & $75.38\%$ & $66.64\%$ & $59.08\%$ & $81.92\%$  & $67.90\%$ & $55.92\%$ & $43.34\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$ & $84.34\%$ & $73.04\%$ & $64.66\%$ & $55.74\%$ & $80.24\%$  & $64.86\%$ & $51.88\%$ & $39.18\%$ \\ \hline \hline
 
\multirow{2}{*}{\makecell{ResNet50 + PNI-A-a-multiply\\ (layerwise)}}
& $\eta \sim \mathcal{N}(0,\sigma^2)$ & $84.04\%$ & $77.26\%$ & $68.96\%$ & $60.52\%$ & $81.20\%$  & $70.30\%$ & $58.26\%$ & $45.96\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$ & $80.56\%$ & $73.96\%$ & $65.76\%$ & $53.60\%$ & $78.34\%$  & $68.94\%$ & $57.78\%$ & $40.20\%$ \\ \hline

\multirow{2}{*}{\makecell{ResNet50 + PNI-A-a-multiply \\ (channelwise)}}
& $\eta \sim \mathcal{N}(0,\sigma^2)$ 
& $84.72\%$ & $76.94\%$ & $69.32\%$ & $61.88\%$ & $81.00\%$  & $70.88\%$ & $59.36\%$ & $46.52\%$ \\ \cline{2-10} 
& $\eta \sim \mathcal{U}(-a,a)$
& $81.12\%$ & $74.90\%$ & $67.80\%$ & $55.54\%$ & $78.74\%$  & $69.44\%$ & $58.54\%$ & $40.02\%$ \\ \hline \hline

\multicolumn{2}{|c||}{\makecell{Iterations per attack}} & x & x & x & x & x & x & x & x \\
\hline
 
\end{tabular}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\label{tab:PNI_variants}
\end{table*}
